MatSwap: Light-aware material transfers in images

We present MatSwap, a method to transfer materials to designated surfaces in an image photorealistically. Such a task is non-trivial due to the large entanglement of material appearance, geometry, and lighting in a photograph. In the literature, material editing methods typically rely on either cumbersome text engineering or extensive manual annotations requiring artist knowledge and 3D scene properties that are impractical to obtain. In contrast, we propose to directly learn the relationship between the input material -- as observed on a flat surface -- and its appearance within the scene, without the need for explicit UV mapping. To achieve this, we rely on a custom light- and geometry-aware diffusion model. We fine-tune a large-scale pre-trained text-to-image model for material transfer using our synthetic dataset, preserving its strong priors to ensure effective generalization to real images. As a result, our method seamlessly integrates a desired material into the target location in the photograph while retaining the identity of the scene. We evaluate our method on synthetic and real images and show that it compares favorably to recent work both qualitatively and quantitatively. We release our code and data on https://github.com/astra-vision/MatSwap

==> latexmkrc <==
#!/usr/bin/perl

#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}



## Put this (Perl) file in the root of your Overleaf project. It overrides the
## `pdflatex` compilation command to run GhostScript as a post-process which will
## compress non-JPEG images to JPEG in the output PDF file. The JPEG quality
## settings are set to high to minimize the loss of image quality. This should
## work well even for images that contain a lot of high-frequency noise.
## To disable, simply rename the file to something other than latexmkrc.
##
## Created by Iliyan Georgiev.

## Quality settings
$PDF_VERSION = 1.4;
$IMG_DOWNSAMPLE = 'true';
$IMG_DOWNSAMPLE_DPI = 600;
$IMG_DOWNSAMPLE_THRESHOLD = 1.0;
$IMG_COMPRESSION_QFACTOR = 0.2;  # lower is better (try 0.08 for higher quality)
$PASSTHROUGH_JPEGS = 'true';

## Don't modify these, they are specified by Overleaf
$GS_INPUT_FILE = '%B.pdf';
$GS_OUTPUT_FILE = '%B-embed.pdf';

## You can try setting below: -dNEWPDF=true
## This fails in the current GhostScript v9.55 on Overleaf 
$GS_COMMAND = "gs
   -sDEVICE=pdfwrite
   -sOutputFile=$GS_OUTPUT_FILE
   -dCompatibilityLevel=$PDF_VERSION
   -dPDFSETTINGS=/default
   -dFastWebView=true
   -dEmbedAllFonts=true
   -dSubsetFonts=true
   -dCompressFonts=true
   -dDetectDuplicateImages=true
   -dDoThumbnails=false
   -dAutoRotatePages=/None
   -dDownsampleColorImages=$IMG_DOWNSAMPLE
   -dColorImageDownsampleType=/Bicubic
   -dColorImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dColorImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleGrayImages=$IMG_DOWNSAMPLE
   -dGrayImageDownsampleType=/Bicubic
   -dGrayImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dGrayImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleMonoImages=$IMG_DOWNSAMPLE
   -dMonoImageDownsampleType=/Subsample
   -dMonoImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dMonoImageResolution=$IMG_DOWNSAMPLE_DPI
   -dConvertCMYKImagesToRGB=true
   -dColorImageFilter=/DCTEncode
   -dGrayImageFilter=/DCTEncode
   -dMonoImageFilter=/CCITTFaxEncode
   -dColorConversionStrategy=/LeaveColorUnchanged
   -dPassThroughJPEGImages=$PASSTHROUGH_JPEGS
   -dProcessColorModel=/DeviceRGB
   -dRenderIntent=1
   -dDefaultRenderingIntent=/Perceptual
   -dUseArtBox
   -dNEWPDF=false
   -dNOPAUSE
   -dBATCH
   -c \"<< /ColorACSImageDict << /VSamples [ 1 1 1 1 ] /HSamples [ 1 1 1 1 ] /QFactor $IMG_COMPRESSION_QFACTOR /Blend 1 /ColorTransform 1 >> >> setdistillerparams\"
   -f $GS_INPUT_FILE";

## Remove new-line characters from GhostScript command
$GS_COMMAND =~ s/\n//g;

## Set the pdflatex command to be used by Overleaf
$pdflatex = "pdflatex %O %S; $GS_COMMAND; mv %B-embed.pdf %B.pdf";

## For debugging
# print "$GS_COMMAND\n";
# print "$pdflatex\n";

